Measurement of forward $J/\psi$ production cross-sections in $pp$ collisions at $\sqrt{s}=13$ TeV

The production of $J/\psi$ mesons in proton-proton collisions at a centre-of-mass energy of $\sqrt{s}=13$ TeV is studied with the \lhcb detector. Cross-section measurements are performed as a function of the transverse momentum $p_\mathrm{T}$ and the rapidity $y$ of the $J/\psi$ meson in the region $p_\mathrm{T}<14\mathrm{GeV}/c$ and $2.0<y<4.5$, for both prompt $J/\psi$ mesons and $J/\psi$ mesons from $b$-hadron decays. The production cross-sections integrated over the kinematic coverage are $15.03\pm 0.03\pm 0.94$ $\mu$b for prompt $J/\psi$ and $2.25\pm 0.01\pm 0.14$ $\mu$b for $J/\psi$ from $b$-hadron decays, assuming zero polarization of the $J/\psi$ meson. The first uncertainties are statistical and the second systematic. The cross-section reported for $J/\psi$ mesons from $b$-hadron decays is used to extrapolate to a total $b\bar{b}$ cross-section. The ratios of the cross-sections with respect to $\sqrt{s}=8$ TeV are also determined.

==> XsectionRatio2D.tex <==
\begin{table}[!tbp]
\caption{\small The ratio of cross-sections between measurements at 13 TeV and 8 TeV in different bins of \pt and $y$
for prompt \jpsi mesons. The systematic uncertainties are negligible.}
\centering
\small
\begin{tabular}{c|ccccc}
\hline
\pt(\gevc)& $2<y<2.5$& $2.5<y<3$& $3<y<3.5$& $3.5<y<4$& $4<y<4.5$\\
\hline
$ 0- 1$&$1.25\pm 0.14  $&$1.24\pm 0.09  $&$1.23\pm 0.08  $&$1.27\pm 0.08  $&$1.30\pm 0.09  $\\
$ 1- 2$&$1.29\pm 0.12  $&$1.28\pm 0.09  $&$1.30\pm 0.08  $&$1.28\pm 0.08  $&$1.39\pm 0.09  $\\
$ 2- 3$&$1.38\pm 0.11  $&$1.35\pm 0.09  $&$1.36\pm 0.08  $&$1.38\pm 0.08  $&$1.39\pm 0.09  $\\
$ 3- 4$&$1.41\pm 0.11  $&$1.43\pm 0.09  $&$1.43\pm 0.09  $&$1.48\pm 0.09  $&$1.56\pm 0.11  $\\
$ 4- 5$&$1.52\pm 0.13  $&$1.44\pm 0.09  $&$1.48\pm 0.09  $&$1.56\pm 0.10  $&$1.62\pm 0.11  $\\
$ 5- 6$&$1.60\pm 0.11  $&$1.58\pm 0.10  $&$1.61\pm 0.10  $&$1.60\pm 0.10  $&$1.76\pm 0.14  $\\
$ 6- 7$&$1.67\pm 0.12  $&$1.56\pm 0.11  $&$1.61\pm 0.11  $&$1.64\pm 0.11  $&$1.80\pm 0.14  $\\
$ 7- 8$&$1.58\pm 0.12  $&$1.53\pm 0.10  $&$1.68\pm 0.12  $&$1.75\pm 0.13  $&$1.87\pm 0.17  $\\
$ 8- 9$&$1.58\pm 0.14  $&$1.64\pm 0.12  $&$1.79\pm 0.14  $&$1.82\pm 0.15  $&$2.02\pm 0.20  $\\
$ 9-10$&$1.71\pm 0.15  $&$1.78\pm 0.14  $&$1.77\pm 0.15  $&$1.90\pm 0.17  $&$2.01\pm 0.25  $\\
$10-11$&$1.76\pm 0.17  $&$1.69\pm 0.14  $&$1.92\pm 0.17  $&$1.94\pm 0.20  $&$2.20\pm 0.32  $\\
$11-12$&$1.94\pm 0.21  $&$1.75\pm 0.18  $&$2.20\pm 0.21  $&$1.68\pm 0.19  $&$2.12\pm 0.36  $\\
$12-13$&$1.76\pm 0.21  $&$1.67\pm 0.17  $&$2.08\pm 0.24  $&$1.96\pm 0.25  $&$2.99\pm 0.60  $\\
$13-14$&$1.75\pm 0.25  $&$1.98\pm 0.25  $&$1.89\pm 0.26  $&$1.40\pm 0.21  $&$5.94\pm 1.57  $\\
\hline
\end{tabular}\label{tab:XsectionRatio2D}
\end{table}


==> XsectionRatio2DFromB.tex <==
\begin{table}[!tbp]
\caption{\small The ratio of cross-sections between measurements at 13 TeV and 8 TeV in different bins of \pt and $y$
for \jpsi-from-$b$ mesons. The systematic uncertainties are negligible.}
\centering
\small
\begin{tabular}{c|ccccc}
\hline
\pt(\gevc)& $2<y<2.5$& $2.5<y<3$& $3<y<3.5$& $3.5<y<4$& $4<y<4.5$\\
\hline
$ 0- 1$&$1.39\pm 0.24  $&$1.38\pm 0.16  $&$1.50\pm 0.19  $&$1.80\pm 0.14  $&$2.24\pm 0.24  $\\
$ 1- 2$&$1.48\pm 0.14  $&$1.52\pm 0.11  $&$1.61\pm 0.11  $&$1.83\pm 0.14  $&$2.07\pm 0.17  $\\
$ 2- 3$&$1.70\pm 0.15  $&$1.54\pm 0.11  $&$1.74\pm 0.11  $&$1.95\pm 0.13  $&$2.04\pm 0.15  $\\
$ 3- 4$&$1.75\pm 0.14  $&$1.64\pm 0.11  $&$1.73\pm 0.11  $&$1.90\pm 0.13  $&$2.35\pm 0.19  $\\
$ 4- 5$&$1.84\pm 0.16  $&$1.77\pm 0.12  $&$1.80\pm 0.12  $&$2.10\pm 0.14  $&$2.50\pm 0.21  $\\
$ 5- 6$&$1.84\pm 0.14  $&$1.82\pm 0.13  $&$1.91\pm 0.13  $&$2.12\pm 0.15  $&$2.35\pm 0.22  $\\
$ 6- 7$&$1.95\pm 0.15  $&$1.90\pm 0.15  $&$2.10\pm 0.15  $&$2.39\pm 0.18  $&$2.80\pm 0.29  $\\
$ 7- 8$&$1.96\pm 0.17  $&$1.89\pm 0.14  $&$2.08\pm 0.16  $&$2.40\pm 0.20  $&$2.59\pm 0.31  $\\
$ 8- 9$&$1.90\pm 0.19  $&$1.93\pm 0.16  $&$2.21\pm 0.20  $&$2.40\pm 0.24  $&$2.35\pm 0.33  $\\
$ 9-10$&$2.03\pm 0.20  $&$1.98\pm 0.18  $&$2.20\pm 0.22  $&$3.19\pm 0.35  $&$4.48\pm 0.89  $\\
$10-11$&$1.93\pm 0.22  $&$2.16\pm 0.21  $&$2.70\pm 0.28  $&$3.10\pm 0.42  $&$4.11\pm 0.79  $\\
$11-12$&$2.33\pm 0.28  $&$2.25\pm 0.26  $&$2.51\pm 0.31  $&$2.73\pm 0.41  $&$6.88\pm 1.64  $\\
$12-13$&$2.02\pm 0.28  $&$1.92\pm 0.23  $&$2.54\pm 0.36  $&$2.48\pm 0.42  $&$5.89\pm 1.65  $\\
$13-14$&$2.54\pm 0.40  $&$2.49\pm 0.35  $&$2.38\pm 0.39  $&$3.55\pm 0.71  $&$2.98\pm 1.04  $\\
\hline
\end{tabular}\label{tab:XsectionRatio2DFromB}
\end{table}


==> XsectionRatioPT.tex <==
\begin{table}[!tbp]
\caption{\small The ratio of cross-sections between measurements at 13 TeV and 8 TeV in different bins of \pt for prompt \jpsi
mesons.  The systematic uncertainties are negligible.}
\centering
\small
\begin{tabular}{ccccccc}
\hline
$0<\pt<1$& $1<\pt<2$& $2<\pt<3$& $3<\pt<4$& $4<\pt<5$& $5<\pt<6$& $6<\pt<7$\\
\hline
"
$1.26\pm 0.09  $&$1.30\pm 0.09  $&$1.37\pm 0.09  $&$1.45\pm 0.09  $&$1.51\pm 0.10  $&$1.61\pm 0.10  $&$1.64\pm 0.10  $\\
$7<\pt<8$& $8<\pt<9$& $9<\pt<10$& $10<\pt<11$& $11<\pt<12$& $12<\pt<13$& $13<\pt<14$\\
\hline
$1.64\pm 0.10  $&$1.71\pm 0.11  $&$1.80\pm 0.12  $&$1.83\pm 0.13  $&$1.92\pm 0.14  $&$1.91\pm 0.15  $&$1.98\pm 0.17  $\\
\hline
\end{tabular}\label{tab:XsectionRatioPT}
\end{table}


==> XsectionRatioPTFromB.tex <==
\begin{table}[!tbp]
\caption{\small The ratio of cross-sections between measurements at 13 TeV and 8 TeV in different bins of \pt for \jpsi-from-$b$
mesons.  The systematic uncertainties are negligible.}
\centering
\small
\begin{tabular}{ccccccc}
\hline
$0<\pt<1$& $1<\pt<2$& $2<\pt<3$& $3<\pt<4$& $4<\pt<5$& $5<\pt<6$& $6<\pt<7$\\
\hline
"
$1.57\pm 0.13  $&$1.63\pm 0.11  $&$1.74\pm 0.11  $&$1.80\pm 0.12  $&$1.90\pm 0.12  $&$1.93\pm 0.12  $&$2.08\pm 0.13  $\\
$7<\pt<8$& $8<\pt<9$& $9<\pt<10$& $10<\pt<11$& $11<\pt<12$& $12<\pt<13$& $13<\pt<14$\\
\hline
$2.06\pm 0.14  $&$2.06\pm 0.14  $&$2.30\pm 0.16  $&$2.38\pm 0.18  $&$2.57\pm 0.21  $&$2.29\pm 0.20  $&$2.60\pm 0.25  $\\
\hline
\end{tabular}\label{tab:XsectionRatioPTFromB}
\end{table}


==> XsectionRatioY.tex <==
\begin{table}[!tbp]
\caption{\small The ratio of cross-sections between measurements at 13 TeV and 8 TeV in different bins of $y$ for prompt \jpsi
mesons.  The systematic uncertainties are negligible.}
\centering
\small
\begin{tabular}{ccccc}
\hline
$2<y<2.5$& $2.5<y<3$& $3<y<3.5$& $3.5<y<4$& $4<y<4.5$\\
\hline
$1.38\pm 0.11  $&$1.36\pm 0.09  $&$1.37\pm 0.08  $&$1.38\pm 0.08  $&$1.44\pm 0.09  $\\
\hline
\end{tabular}\label{tab:XsectionRatioY}
\end{table}


==> XsectionRatioYFromB.tex <==
\begin{table}[!tbp]
\caption{\small The ratio of cross-sections between measurements at 13 TeV and 8 TeV in different bins of $y$ for \jpsi-from-$b$
mesons.  The systematic uncertainties are negligible.}
\centering
\small
\begin{tabular}{ccccc}
\hline
$2<y<2.5$& $2.5<y<3$& $3<y<3.5$& $3.5<y<4$& $4<y<4.5$\\
\hline
$1.68\pm 0.13  $&$1.62\pm 0.10  $&$1.73\pm 0.11  $&$1.96\pm 0.12  $&$2.24\pm 0.15  $\\
\hline
\end{tabular}\label{tab:XsectionRatioYFromB}
\end{table}

